On Minimizing the Impact of Dataset Shifts on Actionable Explanations

The Right to Explanation is an important regulatory principle that allows individuals to request actionable explanations for algorithmic decisions. However, several technical challenges arise when providing such actionable explanations in practice. For instance, models are periodically retrained to handle dataset shifts. This process may invalidate some of the previously prescribed explanations, thus rendering them unactionable. But, it is unclear if and when such invalidations occur, and what factors determine explanation stability i.e., if an explanation remains unchanged amidst model retraining due to dataset shifts. In this paper, we address the aforementioned gaps and provide one of the first theoretical and empirical characterizations of the factors influencing explanation stability. To this end, we conduct rigorous theoretical analysis to demonstrate that model curvature, weight decay parameters while training, and the magnitude of the dataset shift are key factors that determine the extent of explanation (in)stability. Extensive experimentation with real-world datasets not only validates our theoretical results, but also demonstrates that the aforementioned factors dramatically impact the stability of explanations produced by various state-of-the-art methods.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> tables/baseline_shift.tex <==
\begin{table*}[t]
\small 
\centering
\caption{Baseline gradient stability scores for all real-world shifted datasets. The shfit-size column reflects the size of the full, shifted dataset, relative to the original one. (i.e., a value of 1.06 means that if the original dataset contains 100 samples, the shifted version contains 6 additional for a total of 106).  All values average across all test samples and then across all trials. GD is gradient dissimilarity and GA is gradient angle. \anna{not sure where my shap and lime data went. may have to re-run}}
\label{tab:relu_who}
\begin{tabular}{ll|ll|lll|lll}\toprule
                       & Explanation &       &       & \multicolumn{3}{c|}{Top-3} & \multicolumn{3}{c}{Top-5} \\
Shift size                & technique   & GD    & GA    & SA      & CDC    & SSA    & SA      & CDC    & SSA    \\\midrule
\multirow{2}{*}{1.06}   & Saliency    & 0.45 & 0.517 & 0.658 & 0.873 & 0.19 & 0.631 & 0.677 & 0.038 \\
                       & SmoothGrad  & 0.035 & 1.524 & 0.939 & 0.94 & 0.906 & 0.938 & 0.923 & 0.899  \\
                       % & LIME        & 0.336 & 1.260 & 0.357   & 0.173  & 0.143 & 0.375   & 0.137  & 0.133  \\
                       % & K.SHAP      & 0.856 & 1.157 & 0.313   & 0.328  & 0.048 & 0.367   & 0.198  &  0.024 \\
                       \midrule
\multirow{2}{*}{1.33} & Saliency    &    0.419 & 0.543 & 0.641 & 0.851 & 0.184 & 0.617 & 0.632 & 0.034  \\
                       & SmoothGrad  &  0.033 & 1.526 & 0.939 & 0.941 & 0.907 & 0.939 & 0.924 & 0.899 \\
                       % & LIME        & 0.097 &  0.805  & 0.525 & 0.293 & 0.114 &  0.557  &    0.095 &  0.040 \\
                       % & K.SHAP      & 0.614 & 0.769 &  0.486  & 0.680  & 0.157  &  0.538 &  0.561  &  0.080 \\
                       \midrule
\multirow{2}{*}{1.61} & Saliency    & 0.459 & 0.578 & 0.635 & 0.83 & 0.173 & 0.611 & 0.601 & 0.034\\
                       & SmoothGrad  & 0.039 & 1.528 & 0.938 & 0.94 & 0.906 & 0.937 & 0.923 & 0.899\\
                       % & LIME        & 0.031 & 0.334 & 0.892  & 0.710 & 0.701 &  0.921  &  0.688 & 0.688 \\
                       % & K.SHAP      & 0.044 & \textbf{0.248} & 0.835 &  0.830 &  0.550 & 0.837  & 0.570  &  0.370  \\
                       \midrule
\multirow{2}{*}{2.00} & Saliency    & 0.434 & 0.64 & 0.564 & 0.808 & 0.115 & 0.596 & 0.592 & 0.026\\
                       & SmoothGrad  &  0.037 & 1.533 & 0.932 & 0.937 & 0.902 & 0.935 & 0.923 & 0.898 \\
                       % & LIME        & 0.031 & 0.334 & 0.892  & 0.710 & 0.701 &  0.921  &  0.688 & 0.688 \\
                       % & K.SHAP      & 0.044 & \textbf{0.248} & 0.835 &  0.830 &  0.550 & 0.837  & 0.570  &  0.370  \\
                       \bottomrule    
\end{tabular}
\end{table*}



==> tables/metrics.tex <==
\begin{table*}[t]
\small
\centering
\caption{\small Explanation Stability Metrics}
\label{tab:metrics}
\begin{tabular}{lll}\toprule
Metric name & {Metric description}  & Range  \\\midrule
\multirow{3}{*}{SA}  & \textbf{Top-K Sign Agreement} - given the top-k feature sets for two models, what         & \multirow{3}{*}{{[}0,1{]}} \\
     & percent of top-k features appear in both explanations and have the same signed value       &  \\
 & in the gradient? Order of the top-k features does not matter.   &   \\
 \multirow{2}{*}{CDC} & \textbf{Consistent Direction of Contribution} - binary:  do all features in the top-k (for    & \multirow{2}{*}{$\{0,1\}$} \\
   & either model) have the same gradient sign in the other model?  &  \\
  \multirow{3}{*}{SSA} & \textbf{Signed-Set Agreement} - binary: 1 if the two models' top-k feature sets contain      & \multirow{2}{*}{$\{0,1\}$} \\
  & the same features and the features have the same gradient sign. Order of the top-k      &   \\
 & features does not matter. & \\
 % Gradient norm  & Given two sets of gradients $g_1$ and $g_2$, compute $\| g_1 - g_2 \|_2 $                                 & {[}0, $\infty$)            \\
 % \multirow{2}{*}{Gradient angle}    & Given two sets of gradients $g_1$ and $g_2$, return the average angle between entries in     & \multirow{2}{*}{[0, $\pi$]}  \\
 %  & $g_1$ and $g_2$  & \\
\bottomrule
\end{tabular}
\end{table*}
